Towards Robust Off-policy Learning for Runtime Uncertainty

Off-policy learning plays a pivotal role in optimizing and evaluating policies prior to the online deployment. However, during the real-time serving, we observe varieties of interventions and constraints that cause inconsistency between the online and offline settings, which we summarize and term as runtime uncertainty. Such uncertainty cannot be learned from the logged data due to its abnormality and rareness nature. To assert a certain level of robustness, we perturb the off-policy estimators along an adversarial direction in view of the runtime uncertainty. It allows the resulting estimators to be robust not only to observed but also unexpected runtime uncertainties. Leveraging this idea, we bring runtime-uncertainty robustness to three major off-policy learning methods: the inverse propensity score method, reward-model method, and doubly robust method. We theoretically justify the robustness of our methods to runtime uncertainty, and demonstrate their effectiveness using both the simulation and the real-world online experiments.

==> optimization.tex <==
In the reward-maximization setting where the candidate policy is parameterized as $\pi_{\theta} \in \mathcal{F} := \{\pi_{\theta} \, |\, \theta \in \Theta\}$, the minimax training objective in (\ref{eqn:robust-def1}) becomes:
\begin{equation*}
    \underset{\pi_{\theta} \in \mathcal{F}}{\text{maximize}} \min_{\pi_U: e^{-\alpha} \leq \pi_0/\pi_{U} \leq e^{\alpha}} \hat{V}(\pi_{\theta}; \pi_U),
\end{equation*}
Notice that the above objective function can be nonconcave-nonconvex in general, so the Minimax Theorem \citep{sion1958general} does not apply, and the order of $\min$ and $\max$ can not be switched. Therefore, the lower-bounding methods from the previous section, which holds for \emph{any} given $\pi_{\theta}$, play an important role in finding the approximate solution for the minimax problem.
% has important implications. By our design, for each candidate policy $\pi_{\theta}$, the uncertainty in $\pi_U$ behaves adversarially to undermine the off-policy evaluation result for $\pi_{\theta}$. As a consequence, it enforces the robustness of $\pi_{\theta}$ on making prediction under future uncertainty. 
We illustrate how to plug in the lower bounds using the DR estimator as an example, since it includes both the IPS and RM estimator as special cases. 
We use $\hat{V}_{DR}(\pi_{\theta};p,r)$ to denote the objective function for lower-bounding the DR estimator as in (\ref{eqn:optimization-DR}), where $p:=p(a|x)$ and $r:=r(a,x)$ are the optimization policy and reward model, and $\Pi(\pi_0;\alpha)$ and $\mathcal{R}(\pi_0;\alpha)$ give the corresponding constraint sets. It then holds that:
\begin{equation}
\label{eqn:minimax-DR}
\begin{split}
    & \max_{\pi_{\theta} \in \mathcal{F}}\, \min_{e^{-\alpha} \leq \pi_0/\pi_{U} \leq e^{\alpha}} \hat{V}_{\text{DR}}(\pi_{\theta}; \pi_U) \\
    & \geq \max_{\pi_{\theta} \in \mathcal{F}}\, \inf_{p \in \Pi(\pi_0;\alpha), r \in \mathcal{R}(\pi_0;\alpha)} \hat{V}_{DR}(\pi_{\theta};p,r) \\
    & \geq \max_{\pi_{\theta} \in \mathcal{F}} \underline{\hat{V}_{\text{DR}}(\pi_{\theta})}.
\end{split}
\end{equation}
Therefore, we can instead consider optimizing the lower bound of the minimax problem, which leads to a strict non-decreasing optimization path and can be implemented efficiently. In particular, we adopt the minorize-maximization approach described in Algorithm \ref{algo:algo}. We also provide a sketched visual illustration in Figure \ref{fig:optimization} to show the working mechanism. Notice that the constraint sets $\mathcal{R}(\pi_0;\alpha)$ and $\Pi(\pi_0;\alpha)$ do not depend on $\pi_{\theta}$, so we only need to compute them once at the beginning of the optimization. 

\begin{figure}[bht]
    \centering
    \includegraphics[width=0.75\linewidth]{images/optimization.png}
    \caption{\footnotesize A sketched visual illustration for the minorize-maximization optimization procedure.}
    \vspace{-0.4cm}
    \label{fig:optimization}
\end{figure}

\begin{algorithm}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetAlgoLined
\Input{The uncertainty level $\alpha$, history logging policy $\pi_0$, feedback data.}
\Output{The runtime-robust policy $\pi_{\theta^{\text{new}}}$.}
 \textbf{Initialize} $\theta^{\text{new}}$, $p^*$, $r^*$; \\
 Compute the constraints sets $\mathcal{R}(\pi_0;\alpha)$ for RM by solving the auxiliary ERM in Lemma \ref{lemma:apv-eqv}; \\
 Obtain the constraints sets $\Pi(\pi_0;\alpha)$ (second and third line in (\ref{eqn:optimization-DR})); \\
 \While{$\min_{p,r} \hat{V}_{DR}(\pi_{\theta^{\text{new}}}) \geq \min_{p,r} \hat{V}_{DR}(\pi_{\theta^{\text{old}}})$}{
  Let $\theta^{\text{old}} = \theta^{\text{new}}$, compute $\theta^{\text{new}} = \arg \max_{\theta} \hat{V}_{DR}(\pi_{\theta};p^*, r^*)$ using suitable optimization method; \\
  Solve for: $p^*, r^* = \arg \min_{p\in \Pi, r \in \mathcal{R}} \hat{V}_{DR}(\pi_{\theta^{\text{new}}};p, r)$. \\
 }
 \caption{Minorize-maximization procedure for reward optimization}
 \vspace{-0.1cm}
 \label{algo:algo}
\end{algorithm}


From the learning-theoretical perspective, it is important to understand how the proposed approach affects the generalization performance while asserting robustness against runtime uncertainty. Rather than the absolute value of $V(\pi_{\theta})$, we are more interested in the improvement compared with the logging policy: $V(\pi_{\theta}) - V(\pi_0)$. Further, it remains to be examined how does $\alpha$, which controls the asserted robustness in training, affect the generalization.
Towards this end, we first define the Rademacher complexity of a policy class. Let $\epsilon_{i,a}$, $i=1,\ldots,n$, $a \in \mathcal{A}$ be independent Rademacher random variables. Given the feedback data, the empirical Rademacher complexity of $\mathcal{F}$ is given by:
\[\mathcal{R}_n(\mathcal{F}) = \Ebb \sup_{\pi \in \mathcal{F}} \big| \frac{1}{n}\sum_{i=1}^n \sum_{a \in \mathcal{A}} \epsilon_{i,a} \pi(a |x_i) \big|.\]
The Rademacher complexity often has the $\mathcal{O}(1/\sqrt{n})$ rate for common policy classes \citep{mohri2018foundations}. Even for deep learning models, recent work shows that $\mathcal{R}_n(\mathcal{F}) = \mathcal{O}(1/\sqrt{n})$ \citep{bartlett2017spectrally,golowich2018size}.
% Therefore, we assume the same $1/\sqrt{n}$ rate for all the policy classes we consider here. 
In the following theorem, we characterize the generalization of policy improvement under the proposed minorize-maximization algorithm, for any given $\alpha>0$.

\begin{theorem}
\label{thm:main}
Suppose that for all $\alpha>0$, there exists a constant $M_{\alpha}$ such that $\max_{a,x} |\hat{f}_a(x)| \leq M_{\alpha}$ and $\max_{a,x} |\hat{g}_a(x)| \leq M_{\alpha}$. Also, we assume $\pi_0(a|x_i) \in (q, 1-q)$ for some $q>0$. Let $\bar{r} := \max_{i} |r_i|$, then for all $\pi_{\theta} \in \mathcal{F}$ and $\forall \delta > 0$, with probability as least $1-\delta$:
\begin{equation*}
\label{eqn:main}
\begin{split}
     & V(\pi_{\theta}) - V(\pi_0) \geq  \underbrace{\min_{p\in \Pi, r \in \mathcal{R}} \hat{V}_{DR}(\pi_{\theta};p, r) - \hat{V}(\pi_0)}_{\text{I}}  \\
     & \underbrace{- 6\big( \frac{q+1}{q}M_{\alpha} + \bar{r} \big)\sqrt{\frac{2\log \frac{3}{\delta}}{n}}   - 2 \max \big\{M_{\alpha}, \frac{\bar{r}}{q} \big\}\mathcal{R}_n(\mathcal{F})}_{\text{II}},
\end{split}
\end{equation*}
$\hat{V}(\pi_0)$ is the logging policy's value on the training data.
\end{theorem}

The proof is relegated to the appendix. The significance of Theorem \ref{thm:main} is to reveal the two critical components that controls generalization: \emph{I}. the empirical policy improvement under the proposed minorize-maximization algorithm; \emph{II}. the composite terms of the policy complexity and the degree of uncertainty (reflected via $M_{\alpha}$). 

In particular, by enriching $\mathcal{F}$, we are more likely to make \emph{I} positive on training data, but we then suffer from a larger negativity of \emph{II}. This tradeoff is consistent with the standard generalization for supervised learning. More importantly, the magnitude of \emph{II} also increases with $M_{\alpha}$. Notice that $M_{\alpha}$ is often non-decreasing in $\alpha$ as the RM bounds get more loose (see Figure \ref{fig:lower-bounds} for illustration). As a consequence, having $\alpha>0$ further penalizes the model complexity and the slack term in \emph{II}, so increasing $\alpha$ will encourage the algorithm to select the policy that achieves less empirical improvement but has smaller complexity. This explains from the theoretical perspective how our approach can lead to policy that performs better under runtime uncertainty. To summarize, the result in Theorem \ref{thm:main} shows rigorously how and why introducing $\pi_U$ with $e^{-\alpha} \leq \pi_0/\pi_{U} \leq e^{\alpha}$ can improve the robustness of the learnt policy.
% while a larger $\alpha$ asserts more robustness to the optimized policy, it makes the empirical improvement on the training data more difficult to generalize. Therefore, Theorem \ref{thm:main} also characterizes the tradeoff between pursing robustness and achieving more improvement during our off-policy learning. 

% In particular, 
% the empirical improvement can always be made positive if $\min_{p\in \Pi, r \in \mathcal{R}} \hat{V}_{DR}(\pi_{\theta};p, r) - \hat{V}(\pi_0) \geq 0$ when $n$ is large (so the impact of \emph{II} diminishes). Recall that $\pi_0 \in \Pi$ by the definition, so the true reward model is likely to be bounded in $\mathcal{R}$ under our construction. Therefore, to make \emph{I} positive, we enrich $\mathcal{F}$ such that it includes the logging policy. 

% On the other hand, the magnitude of \emph{II} increases with the complexity $\mathcal{R}_n(\mathcal{F})$ and $M_{\alpha}$. Notice that $M_{\alpha}$ is often non-decreasing in $\alpha$, because under a larger uncertainty, the bounds are more conservative (as shown in Figure \ref{fig:lower-bounds}) and have a larger infinity norm. So the negativity of \textbf{II} also increases with $\alpha$. 

% \begin{itemize}
%     \item The empirical improvement in \textbf{I} can always be made possible if $\min_{pi\in \Pi, r \in \mathcal{R}} \hat{V}_{DR}(\pi_{\theta};\pi, r) - \hat{V}(\pi_0) \geq 0$ and $n$ is large enough (so the negative impact of \textbf{II} diminishes). Notice that we have $\pi_0 \in \Pi$ by definition, and are very likely to have the true reward model in $\mathcal{R}$ by our construction. Therefore, to make \textbf{I} positive, we may enrich $\mathcal{F}$ such that it covers the history logging policy.
%     \item The magnitude of \textbf{II} increases with the complexity $\mathcal{R}_n(\mathcal{F})$ and $M_{\alpha}$. Notice that $M_{\alpha}$ is often non-decreasing in $\alpha$, because under a larger uncertainty, the bounds are more conservative (as shown in Figure \ref{fig:lower-bounds}) and have a larger infinity norm. So the negativity of \textbf{II} also increases with $\alpha$. 
% \end{itemize}

% We conclude from the above arguments the tradeoff between prediction robustness and policy improvement. If we are conservative and use a large $\alpha$, the learnt policy will be more robust under future uncertainty, but is less likely to improve upon the past policy due to stronger perturbations in training. Also, with a richer policy class, we are more likely to end up with a robust selection; however, the increased complexity will make the training difficult and thus requires more data.


